Extending OCaml's 'open'

We propose a harmonious extension of OCaml's 'open' construct. OCaml's existing construct 'open M' imports the names exported by the module 'M' into the current scope. At present 'M' is required to be the path to a module. We propose extending 'open' to instead accept an arbitrary module expression, making it possible to succinctly address a number of existing scope-related difficulties that arise when writing OCaml programs.

==> eptcsdata.tex <==
\providecommand{\firstpage}{1}
\providecommand{\publicationstatus}{Sam Lindley and Gabriel Scherer (Eds.):\\
ML Family / OCaml Users and Developers workshops 2017\\
EPTCS 294, 2019, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.294.1}{10.4204/EPTCS.294.1}}

